Sequential Change Point Detection for PSK Modulation Switching

Transmitters in adaptive communication systems may switch their modulation scheme at an unknown time, and a receiver must detect this switch quickly without raising frequent false alarms. Existing modulation classification methods label a finite block of received data and do not provide stopping rules with controlled false-alarm and delay performance. We study the sequential detection of a switch from one phase shift keying (PSK) scheme to another over an additive white Gaussian noise channel. We build cumulative-sum (CUSUM) and moving-sum (MOSUM) detectors from the log-likelihood ratio and its low-SNR approximation. For a switch from quadrature PSK to binary PSK, we derive the moment-generating function and probability density function of the approximate statistic. We use them to relate the CUSUM threshold to the average run length to false alarm and the worst-case detection delay. For a switch between any two PSK orders, we approximate the vector of overlapping MOSUM statistics as multivariate Gaussian and obtain bounds on both measures. Monte Carlo simulations show that our derived expressions for ARL2FA and WADD closely match the empirical results across thresholds, validating the accuracy of the proposed analytical approximations and theoretical bounds.

==> Figures/Dummy_figure.tex <==
\pgfplotsset{axis_Pd_SNR_n_15/.style=
{
	      width=10cm,
 	      legend style={at={(0.3,0.25)},anchor=west},
        ylabel={\footnotesize{$P_D$}},
	      xlabel={\footnotesize{$SNR$}},
	      xmin=-3,xmax=10,
	      ymin=0,ymax=1,
	      grid=both,
	      xtick={-3, -1.5, 0, 1.5, 3, 4.5, 6, 7.5, 9},
 	      ytick={0,0.2,0.4,0.6,0.8,1},
	      xticklabels={\scriptsize{-3}, \scriptsize{~}, \scriptsize{0}, \scriptsize{~}, \scriptsize{3}, \scriptsize{~}, \scriptsize{6}, \scriptsize{~}, \scriptsize{9}}},
	      yticklabels={\scriptsize{0},\scriptsize{0.2},\scriptsize{0.4},\scriptsize{0.6},\scriptsize{0.8},\scriptsize{1}}
}
%-----------------------------------------
\begin{tikzpicture}

\begin{axis}[axis_Pd_SNR_n_15]
% 
%--------------------------------------------
% 1: No processing
%
\addplot [color = green, very thick, mark=o, mark options={solid}, mark size=2pt] coordinates  {
% 
(-3,0.3)
(-1.5,0.35)
(0,0.42)
% (1.5,)
(3,0.76)
(5, 0.86)
% (7.5, )
(10, 0.94)
};
% 
% %--------------------------------------------
% 2a: Tanh processing
% %
\addplot [color = red, very thick, dashed, mark=x, mark options={solid}, mark size=2.2pt] coordinates  {
%
(-3,0.1)
% (-1.5,0.35)
(0,0.23)
% (1.5,)
(3,0.46)
% (5, 0.86)
% (7.5, )
(10, 0.92)
};
% %
% %--------------------------------------------
% 2b: Tanh LLR processing
% %
\addplot [color = black, very thick, mark=*, dotted, mark options={solid}, mark size=1.8pt] coordinates  {
% %
(-3,0.3)
(-1.5,0.35)
(0,0.42)
% (1.5,)
(3,0.76)
(5, 0.86)
% (7.5, )
(10, 0.94)
};
% %
% \legend{\scriptsize{No processing}, \scriptsize{Tanh processing}, \scriptsize{tanh LLR processing}}
% %
\end{axis}
%
% \draw [thick, fill=white] (1-0.2,0.05) rectangle(3,1.1);
%
% \draw [-, very thick, blue] (1.2-0.2,0.9) -- (1.2+0.6-0.2,0.9);
% \draw [very thick, blue] (1.2-0.2+0.3,0.9) circle (0.07);
% \node [right] at (1.2+0.6-0.2,0.9){\scriptsize{$p=0.001$}};
%
% \draw [-, very thick, red, dashed] (1.2-0.2,0.9-0.3) -- (1.2+0.6-0.2,0.9-0.3);
%
% \draw [-, very thick, red] (1.2-0.2+0.3-0.06,0.9-0.3+0.06) -- (1.2-0.2+0.3+0.06,0.9-0.3-0.06);
% \draw [-, very thick, red] (1.2-0.2+0.3+0.06,0.9-0.3+0.06) -- (1.2-0.2+0.3-0.06,0.9-0.3-0.06);
%
%
% \node [right] at (1.2+0.6-0.2,0.9-0.3){\scriptsize{$p=0.01$}};
%
% \draw [-, very thick, dotted] (1.2-0.2,0.9-0.6) -- (1.2+0.6-0.2,0.9-0.6);
% \draw [very thick, fill=black] (1.2-0.2+0.3,0.9-0.6) circle (0.07);
% \node [right] at (1.2+0.6-0.2,0.9-0.6){\scriptsize{$p=0.03$}};
%
% %----------------------------------
% \node [below] at (1.5,-0.8){\scriptsize{(c) Inner.~prod.~pre-processing}};
    
\end{tikzpicture}


==> Figures/combined_CUSUM_MOSUM_analysis.tex <==


\begin{figure*}[!t]
    \centering

    %================ CUSUM: top two plots ================
    \begin{minipage}{0.95\textwidth}
        \centering
        \begin{minipage}{0.48\textwidth}
            \centering
            \input{Figures/cusum/ARL2FA_results}
        \end{minipage}
        \hfill
        \begin{minipage}{0.48\textwidth}
            \centering
            \input{Figures/cusum/WADD_results}
        \end{minipage}

        \captionof{figure}{$ARL2FA$ and $WADD$ versus threshold
        for the QPSK-to-BPSK CUSUM at SNR = 2~dB.}
        \label{fig:Bounds_CUSUM}
    \end{minipage}

    \vspace{0.8cm}

    %================ MOSUM: bottom two plots ================
    \begin{minipage}{0.95\textwidth}
        \centering
        \begin{minipage}{0.48\textwidth}
            \centering
            \input{Figures/MOSUM_w=100_ARL2FA_Bounds}
        \end{minipage}
        \hfill
        \begin{minipage}{0.48\textwidth}
            \centering
            \input{Figures/MOSUM_w=100_WADD_Bounds}
        \end{minipage}

        \captionof{figure}{Theoretical bounds and empirical values of
        $ARL2FA$ and $WADD$ for MOSUM with $w=100$, for the
        8-PSK-to-BPSK transition at SNR = 2~dB.}
        \label{fig:Bounds_MOSUM}
    \end{minipage}

\end{figure*}

==> Figures/window_effect/window_effect.tex <==
% Requires:
% \usepackage{pgfplots}
% \pgfplotsset{compat=1.18}

\begin{tikzpicture}
\begin{axis}[
    width=\columnwidth,
    height=5.2cm,
    xmode=log,
    ymode=log,
    xmin=1e-4,
    xmax=1,
    ymin=20,
    ymax=2000,
    xlabel={$P_{\mathrm{FA}}$},
    ylabel={ADD},
    grid=major,
    grid style={dotted,gray!50},
    legend pos=north east,
    legend style={font=\scriptsize,draw=none,fill=white},
    tick label style={font=\scriptsize},
    label style={font=\small},
    mark size=1.7pt,
    line width=0.7pt,
]

% w = 30
\addplot+[blue,mark=*] coordinates {
    (0.0020,1875.165)
    (0.0058,774.935)
    (0.0121,522.706)
    (0.0558,264.331)
    (0.1034,195.085)
    (0.3325,112.694)
    (0.7442,72.377)
};
\addlegendentry{$w=30$}

% w = 60
\addplot+[red,mark=square*] coordinates {
    (0.0003,280.813)
    (0.0018,144.996)
    (0.0054,112.461)
    (0.0151,90.266)
    (0.0419,74.951)
    (0.1026,64.623)
    (0.7730,47.964)
};
\addlegendentry{$w=60$}

% w = 100
\addplot+[orange!80!black,mark=triangle*] coordinates {
    (0.0002,101.905)
    (0.0010,95.089)
    (0.0037,84.924)
    (0.0094,81.031)
    (0.0446,74.294)
    (0.0912,71.212)
    (0.7507,59.060)
};
\addlegendentry{$w=100$}

\end{axis}
\end{tikzpicture}

==> Individual_Files/Section_7_Future_Plots.tex <==
Simulations setup
Number of trials = $10^5$

number of  samples : 
\begin{itemize}
\item WADD - only post change $(10^5)$
\item ADD - pre and post change ($10^3$ pre, $10^5$ post)
\item PFA - only pre change ($10^4$)
\item  * bounds verification is only post changethat 
\item values of SNR 
\item +/- { (5, 4, 3, 2, 1, 0)} decibles
\item  +2 DB for common graphs
\end{itemize}

Six methods

\begin{enumerate}
\item G:Exact CUSUM
\item G:Approximate CUSUM
\item G:K-CUSUM
\item D:Exact MOSUM 
\item D:Approx MOSUM 
\item D:Cumulant MOSUM
\end{enumerate}

\vspace{0.1in}


\begin{itemize}
%
\item \tcr{PFA vs ADD: 5 methods.. fixed SNR=2dB.. fixed window=100 for MOSUM}
%
\begin{itemize}
\item \tcr{Fig.1.1: QPSK to BPSK} \tcb{ready}
\item \tcr{Fig.1.2: 16-PSK to 8-PSK} \tcb{Priority-3}
\item Fig.1.3: 64-PSK to 32-PSK
\end{itemize}
%
\item \tcr{ADD vs SNR} .. 5 methods.. fixed PFA=0.1.. fixed h .. fixed window for MOSUM.. fixed w for all SNRs
%
\begin{itemize}
\item Fig.2.1: QPSK to BPSK
\item \tcr{Fig.2.2: 16-PSK to 8-PSK} \tcb{Priority-1}
\item Fig.2.3: 64-PSK to 32-PSK
\end{itemize}
%
\item Effect of window...Exact MOSUM, Approx MOSUM, Cumulant MOSUM ... plot PFA vs ADD.. fixed SNR
%
%
\begin{itemize}
\item \tcr{Fig.3.1: QPSK to BPSK}
\tcb{Priority-2}
\item Fig.3.2: 16-PSK to 8-PSK
\item Fig.3.3: 64-PSK to 32-PSK
\end{itemize}
%
\item Effect of PSKs: QPSK to BPSK, 16-PSK to QPSK, 64-PSK to 32-PSK.. fix SNR.. pltos PFA vs ADD.. Ideally all 6 methods
%
\begin{itemize}
\item Fig.4.1: Approx CUSUM
\item Fig.4.2: Aprrox MOSUM
\end{itemize}
%
%
\end{itemize}


%\cref{fig:Bounds_MOSUM} shows that, for \(w=100\) and an \(8\)-PSK to BPSK transition at \(2\) dB SNR, the proposed analytical bounds closely track the simulated performance over the investigated threshold range. We get the plot for $ARL2FA_{MC}$ and $WADD_{MC}$ by running the MOSUM algorithm over a sufficiently large sequence of $N$ symbols and calculating the average stopping time for the algorithm using different thresholds $h_m^\lambda$. For $ARL2FA$, the Monte Carlo results remain consistently between the lower bound $L_{\scriptscriptstyle{M}}$ and the upper bound $U_{\scriptscriptstyle{M}}$, with the three curves exhibiting the same increasing trend as the threshold \(h_m^\lambda\) increases. A similar behavior is observed for WADD, where the simulated detection delay is bounded by $L_{\scriptscriptstyle{M^{\prime}}}$ and $U_{\scriptscriptstyle{M^{\prime}}}$ across the entire threshold range. The relatively narrow separation between the bounds indicates that the Gaussian approximation provides a useful characterization of the MOSUM performance for this setting.

%For practical analysis of bounds, the multivariate normal CDFs required for evaluating the non-exceedance probabilities $\kappa_{\scriptscriptstyle{M},w}$ and $\rho_{\scriptscriptstyle{M},w}$ were computed numerically using the \texttt{multivariate\_normal.cdf} routine from the Python SciPy library.



==> stray_files/Meeting_summary.tex <==
========================================\\
1-Feb-2026: Next meeting to do list: 
 
\begin{itemize}
%
\item Recreate Fig. 3(a) from 1995 paper + 1991 paper
\item Davin: Finish window based simulations
\item Guneesh: Read 1995 paper
\item Davin: Find 5 good feature based papers: Main focus
%    
\end{itemize}

========================================\\
10-Feb-2026: Next meeting to do list: 
 
\begin{itemize}
%
\item Davin: LRT: Recreate Fig. 3(a) from 1995 paper + 1991 paper \tcr{Done}
\item Davin: FB: Implement 2000 paper.. cumulant paper.. PSK to QPSK \tcr{Done}
\item Davin: Read 2015 Sequential detection paper + implement it + Choose 2000 paper feature
\item Davin: To discuss one more FB paper \tcr{Done}
\item Davin: To add 10 LB papers + 10 FB papers to spreadsheet.. after 2005
\item Guneesh: Read 1995 paper 
\item Guneesh: Read one more ~2015 paper on modulation classification.. non-ML
%    
\end{itemize}

========================================\\
17-Feb-2026: Next meeting to do list: 
 
\begin{itemize}
%
\item Read 2015 Sequential detection paper + implement it
%
\item Read: 1995, 2000 paper Performance analysis: We need distributions of qM and c42
%
\item Read about Hilbert transform: B K Dey lectures
%
\item Finish simulations: Effect of window, effect of h, effect of SNR: Plot E(Delay), E(FA)
\begin{itemize}
\item Using LR 1995 paper
\item Using FB 2000 cumulant paper
\item Using FB 2008 power spectrum based paper
\end{itemize}
%
\item Plot categories:
\begin{itemize}
\item Effect of window w 
\item effect of h
\item effect of SNR
\end{itemize}
%
\item Simulation for offline setup as well
%
\item Find one more feature based paper whose distribution is characterized analytically
%    
\end{itemize}


========================================\\
2-March-2026: Next meeting to do list: 
 
\begin{itemize}
%
\item \tcr{Guneesh + Davin: Read sequential 2015 paper. VVIMP.. check thesis}
%
\item Davin: Finish structure of the main code.. Algo1:LRT, Algo2:C42, take of threshold.. no manual entries..import from csv/json.. correct calculation for False alarm, delay in detection
\item Davin: Start reading performance analysis for all methods
\item Guneesh: Search a good paper feature based paper + implement it.. classification. Ash Davin which paper? Power spectrum.. read performance analysis as well
\item Guneesh + Davin: Think P(FA) calculations if correct classification probabilities are known
%    
\end{itemize}

========================================\\
10-March-2026: Next meeting to do list (Davin): 

\begin{itemize}
\item Finish simulations 
\begin{itemize}
\item Check SNR plot.. vary choice of h
\item FB 2000 cumulant
\item FB 6th order cumulant
\end{itemize}
\item 2015 sequential detection paper
\item Finalize FB based for our implementation: 2000, 2015, 2020
\item Think P(FA) calculations if correct classification probabilities are known
\end{itemize}

%=========================
\section{Our method}

Davin:

\begin{itemize}
\item Method-1: LR 1995
\item Method-2: C42:
\item Method-3: Power spectrum
\item Method-4: ?
\item Method-5: ?
\item Method-6: ?
\end{itemize}

==> stray_files/System_model.tex <==

\input{Figures/Figure_System_model_CPD_Online_M1M2}

In this work, we consider a setup where the transmitter uses the phase shift keying (PSK) modulator and at some unknown time instance $\tau$ it switches from $M'$-PSK to $M$-PSK  (see \cref{Figure_system_model_M1M2}). 
%
Let $s_k^{\prime}(t)$ and $s_k(t)$ denote the modulated waveforms corresponding to the $k$-th symbol index for $M'$-PSK and $M$-PSK respectively.
%
As illustrated in the figure, $s_1^{\prime}(t), s_2^{\prime}(t), \ldots,  s_{\tau}^{\prime}(t)$ denote the waveforms corresponding to $M^{\prime}$-PSK and $s_{\tau+1}(t), s_{\tau+2}(t), \ldots $ denote the waveforms corresponding to $M$-PSK. We consider the passband signal based model for the PSK modulation and assume that 
the noise is introduced by the
additive white Gaussian noise (AWGN) channel
to get the received waveforms $r_1(t),  \ldots,  r_{\tau}(t), r_{\tau+1}(t), \ldots$.
%
The goal is to estimate the change-point location, denoted by $\hat{\tau}$, where the switch between modulation schemes happen. We formulate and solve this problem as a \textit{sequential change-point detection (CPD)} problem~\tcr{(cite CPD book)}.

For the $k$-th symbol index, the transmitted waveform $s_k(t)$ corresponding to $M$-PSK is given by~(\tcr{cite any std digi comm book})
%
\begin{equation}
    s_k(t)
    =
    \operatorname{Re}
    \left\{
        \sqrt{2S}\,
        e^{j\theta_k}
        p(t-(k-1)T_s)
        e^{j(2\pi f_c t+\theta_c)}
    \right\},
\end{equation}
%
where $S$ denotes the signal power, $T_s$ is the symbol duration, $p(t)$ is the transmit pulse, $\theta_c$ is the known carrier phase, and $\theta_k$ denotes the phase of the $k$-th symbol.
%
For $M$-PSK, the information-bearing phase $\theta_k$ is given by
%
\begin{equation}
    \theta_k \in
    \left\{
        \frac{2\pi m}{M}
        : m=0,\ldots,M-1
    \right\}.
\end{equation}
%
The expressions for the waveform of $M^{\prime}$-PSK can be written in a similar manner. 
%and for the setup of \cref{Figure_system_model_M1M2}, the transmitted waveform $s(t)$ will be given by
%
%\begin{align}
%s(t) = \sum_{k=1}^{\tau} s_k^{\prime} (t) + \sum_{k=1}^{\infty} s_k (t).    
%\end{align}
%
The received signal $r_k(t)$ corresponding to the $k$-th symbol is given by
%
\begin{equation}
%
r_k(t) = 
\begin{cases} 
s_k^{\prime}(t) + n_k(t),     & \text{if } k \leq \tau \\
s_k(t) + n_k(t),     & \text{if } k > \tau ,
\end{cases}
%
\end{equation}
%
where $n_k(t)$ denote zero-mean AWGN with a two-sided power spectral density of $N_0/2$ W/Hz. Let $\gamma_s$ denotes the symbol signal-to-noise ratio (SNR), given by
%
\begin{equation}
\gamma_s = \frac{S T_s}{N_0}.
\label{eq:snr_def}
\end{equation}




Let $l_{MPSK}$ and $l_{M^{\prime}PSK}$ denote the log likelihood of receiving $r_k(t)$ under the condition $M$-PSK and $M^{\prime}$-PSK are used respectively. It is known that~{cite 1995 paper}, $l_{MPSK}$ is given by
%
\begin{align}
%
l_{MPSK}^k &\coloneqq \log \mathbb{P} \big[r_k(t)|M)\big] \\
&=  \mbox{~eq. (4) 1995},
%
\end{align}
%
where $\tilde{r}_k$ denote the normalized complex-valued observation obtained after down-conversion, pulse-matched filtering, and symbol-rate sampling, given by~\tcr{cite digi comm book, 1995 paper}
%
\begin{align}
\tilde{r}_k =     .
\end{align}
%
Let $\ell_k$ denote log likelihood ratio (LLR) of receiving $r_k(t)$ given by 
%
%
\begin{align}
\ell_k \coloneqq \log \frac{[r_k(t)|M]}{[r_k(t)|M^{\prime}]} = l_{MPSK}^k - l_{M^{\prime}PSK}^k.
\end{align}
%
\tcr{Discuss approximation..1995 paper.. when applicable.. when..$M^{\prime} > M$ etc}
%
\begin{align}
\ell_k \approx \lambda_k &= \lambda_{M^{\prime}PSK} -  \lambda_{MPSK}\\
&= \Re\left\{ (\tilde{r_k})^M \right\},
\end{align}
%
where $\Re \{\cdot \}$ denote .... \tcr{define a macro for $\Re\left\{ (\tilde{r_k})^M \right\}$.. it will be used at many places}


\tcr{=====Edited till this point====}

Let $\tilde{r}_k$ denote the normalized complex-valued observation obtained after down-conversion, pulse-matched filtering, and symbol-rate sampling. It is given by~\tcr{cite digi comm book}
%
\begin{equation}
  \tilde r_k = \sqrt{2\gamma_s}\, e^{j\theta_k} + n_k, \qquad
  n_k \sim \mathcal{CN}(0, 1),
  \label{eq:observation_model}
\end{equation}
where $n_k$ is a normalized complex Gaussian noise sample, independent
across $k$
%
\cref{eq:observation_model} is the
baseband quantity that all subsequent detection statistics operate on.


The phase $\theta_k$ is determined by the underlying PSK modulation
scheme. Therefore, a change in the modulation order results in a change
in the distribution of the received observations. Specifically, suppose
that at an unknown change point $\tau$, the modulation changes from
$M'$-PSK to $M$-PSK. The observation sequence then follows the
pre-change distribution $P_0$ before $\tau$ and the post-change
distribution $P_1$ from $\tau$ onward: \tcr{not correct}
\begin{equation}
    \tilde{r}_k \sim
    \begin{cases}
        P_0, & k < \tau,\\
        P_1, & k \geq \tau.
    \end{cases}
    \label{eq:change_point_model}
\end{equation}


% At an unknown change point $\tau$, modulation order of the
% received signal changes from $M'$-PSK to $M$-PSK.
% Accordingly, the distribution of the observation sequence changes from
% pre-change distribution $P_0$ to post-change distribution $P_1$,
% such that
% \begin{equation}
%     \tilde{r}_k \sim
%     \begin{cases}
%         P_0, & k < \tau,\\
%         P_1, & k \geq \tau.
%     \end{cases}
% \end{equation}

This change point $\tau$ is unknown, and the detector processes the
observations sequentially to detect its occurrence as quickly as
possible while controlling the false alarm probability.
For the binary hypothesis test between $M$-PSK and $M'$-PSK, the
optimal decision rule is obtained from the difference between the
corresponding log-likelihood functionals (LLFs)
\cite{huang1995likelihood}. Accordingly, for the sequential
change-point formulation, we define the per-observation log-likelihood
ratio as \tcr{not correct}
\begin{equation}
    \ell_k
    =
    \log
    \frac{p(\tilde{r}_k;P_1)}
         {p(\tilde{r}_k;P_0)},
\end{equation}
where $P_0$ and $P_1$ denote the pre-change and post-change
distributions, respectively.

The change-point detection problem is therefore to determine based on
the sequentially observed samples $\tilde{r}_1,\tilde{r}_2,\ldots$,
whether and when the underlying distribution has switched from $P_0$
to $P_1$. We need to find a stopping time $T$, that declares a change as soon as possible
after $\tau$ while keeping the rate of false alarms (declaring a change when none has occurred) acceptably low. 

\tcb{While $\ell_k$ in principle characterizes the full information
available in a single observation, evaluating it exactly is theoretically difficult.} In Section~III, we specialize
to the case $M'>M$, and use a tractable low-SNR approximation to $\ell_k$ that is used to construct two sequential detectors.

==> stray_files/Windowed_CUSUM.tex <==
To detect the transition from $M$-PSK to $M'$-PSK, a one-sided
CUSUM recursion is employed.

\begin{algorithm}
\caption{Windowed CUSUM Detector}

$Z_0 \gets 0$\;

\For{$k=1,2,\ldots$}{

     Compute q_k;
     
    $Z_k \gets \max(0,Z_{k-1}+q_k-\delta)$\;

    \If{$Z_k > c$}{
        Declare modulation change\;
        $T_{\mathrm{det}} \gets k+w$\;
        
        \Return{$\tau_{\mathrm{det}}$}\;
    }
}
\end{algorithm}


A change is declared when the statistic exceeds a
prescribed threshold $c$, yielding the stopping time

\begin{equation}
\tau_{\mathrm{det}}
=
\inf
\left\{
k \ge 1 :
Z_k > c
\right\}.
\label{eq:stopping_time}
\end{equation}

The threshold $c$ controls the trade-off between false alarms and
detection delay. Larger values of $c$ increase the average run length
to false alarm but result in slower detection of the modulation-order
change.

